Spatio-Temporal Ranked-Attention Networks for Video Captioning

Generating video descriptions automatically is a challenging task that involves a complex interplay between spatio-temporal visual features and language models. Given that videos consist of spatial (frame-level) features and their temporal evolutions, an effective captioning model should be able to attend to these different cues selectively. To this end, we propose a Spatio-Temporal and Temporo-Spatial (STaTS) attention model which, conditioned on the language state, hierarchically combines spatial and temporal attention to videos in two different orders: (i) a spatio-temporal (ST) sub-model, which first attends to regions that have temporal evolution, then temporally pools the features from these regions; and (ii) a temporo-spatial (TS) sub-model, which first decides a single frame to attend to, then applies spatial attention within that frame. We propose a novel LSTM-based temporal ranking function, which we call ranked attention, for the ST model to capture action dynamics. Our entire framework is trained end-to-end. We provide experiments on two benchmark datasets: MSVD and MSR-VTT. Our results demonstrate the synergy between the ST and TS modules, outperforming recent state-of-the-art methods.

==> background.tex <==
\section{Notation and Preliminaries: Temporal Attention}
\label{sec:background}
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm,trim={4.4cm 3.5cm 9.8cm 7cm},clip]{./figs/attention_model.pdf}
    \caption{Standard temporal attention model for video captioning.}
    \label{fig:att_model}
\end{figure}
In this section, we introduce our notation and review prior temporal attention models on which we build our STaTS framework. Suppose we are given a training set of $N$ videos,  $\mathfrak{S}=\set{(\seq_1,\capt_1), (\seq_2,\capt_2), \cdots, (\seq_N, \capt_N)}$. Here, $\seq_k$ is a temporally ordered sequence of frame-level features for video $k$, and each $\capt_k$ is a textual description of the video (caption), the words of which are encoded using their indices in a predefined dictionary. Let each video sequence $\seq_k=\langle \vx_1, \vx_2, \cdots, \vx_T\rangle$ be a sequence of $T$ temporally ordered video frames.\footnote{For notational convenience, we assume that all videos have $T$ frames and all sentences have $m$ words. However, we do not make any such assumption in our implementation.}  Illustratively, suppose we feed-forward each frame in a video sequence through a deep convolutional neural network (CNN) and extract the features from a fully-connected layer (e.g., the fc6 layer in a VGG\nobreakdash-16 network). Then, $\vx_t$ is a $d$-dimensional feature vector that captures the visual data of frame $t$. To encode captions, we assume each $\capt_k=\langle \vy_1, \vy_2, \cdots, \vy_{m}\rangle$ is an ordered sequence of word embeddings, where the $i$th word in the caption, $\vy_i \in \binary{D},$ is a one-hot vector encoded using a language dictionary of size~$D$.
%and each such $\sX^t$ be a set of $n$ frame-level features, i.e., $\sX^t = \set{\vx^t_1, \vx^t_2, \cdots, \vx^t_n}$, each $\vx\in\reals{d}$.

Using the notation above, a video caption generation model can be written as a function $f:\reals{d\times T}\to\binary{D\times m}$ that maps the video features into a sequence of words. Figure~\ref{fig:att_model} provides a high-level overview of our discussion to follow. Given that the size of the language dictionary $D$ is usually enormous, learning such a mapping function $f$ could be technically challenging (as the space of sentences is of size $D^m$). Fortunately, however, the language model is highly structured and compositional. As a result, instead of generating all the words in a sentence at once, one could generate each word sequentially conditioned on the previously generated words (thereby reducing the search space to size $mD$). To encode the sentences, a long short-term memory (LSTM) network is typically used, which takes as input the current word $\vy_i$ in a sentence $\capt_k$ and a state representation $h_{i-1}$ of the previous words in the sentence, and produces a new state as output: $h_i = \lstm(h_{i-1}, \vy_i)$. Using a representation of visual features, say $\hat{x}$ (which we discuss in a moment), one could predict the next word in a caption as:
\begin{equation}
  \hat{\vy}_i = \onehot \big( \softmax \big(g(h_{i-1}, \hat{x})\big)\big), 
  \label{eq:1}
\end{equation}
where $g$ is a parameterized non-linear function that combines the LSTM language representation $h$ and the visual feature $\hat{x}$, producing a score for each word in the dictionary. The $\softmax$ function converts the score to a probability vector over the $D$-dimensional dictionary, from which the most probable word is selected using the $\onehot$ function. To learn the parameters of the LSTM and the function $g$ (which could itself be a deep neural network), the predicted $\hat{\vy}_i$ vector is compared to the ground truth word via the cross-entropy loss. During testing, the word with the highest probability is selected.

While the sequential compositionality of the language model enables tractable inference for the language model, such a scheme might not be appropriate for the temporally ordered visual features. Instead, one could use the language model to attend to specific visual features in order to generate the next word in the caption. This is the (by now) standard \emph{temporal attention} model, which uses an attention sub-module to score each visual feature's usefulness for predicting the next word in the caption. Mathematically, let $\ve\in\simplex{T}$ be a probability vector in the $T$-dimensional simplex; its $t$th dimension $\ve_t$ captures the probability that visual feature $\vx_t$ is useful for generating the $i$th word. Typically, $\ve_t$ is given by:
\begin{equation}
\ve_t = \softmax\left(\att\left(h_{i-1}, \vx_t\right)\right),
\label{eq:2}
\end{equation}
where $\att$ is a suitable nonlinear attention function, usually chosen as 
\begin{equation}
\att(h_{i-1}, \vx_t)=\vw^{\mathrm T}\tanh\left(\mW_h h_{i-1} + \mW_x\vx_t + \bias\right).
\label{eq:attn}
\end{equation}
Here, $\bias$ is a learned bias, while $\mW_h$ and $\mW_x$ are learned matrices transforming the respective features into an attention space, in which they are linearly combined using the $\vw$ vector after passing through the non-linear $\tanh$ function. The score $\ve$ is projected onto the simplex via the $\softmax$ operator, thereby generating a probability vector over the visual features. The $\ve$ vector is then used to generate a temporally-attended feature vector as:
\begin{equation}
\hat{x} = \sum_{t=1}^T \ve_t \vx_t,
\label{eq:3}
\end{equation}
which is used in~\eqref{eq:1} above. Note that as the generated caption evolves, the corresponding LSTM state vector $h$ in~\eqref{eq:2} allows the attention module to focus on suitable visual features for generating the next caption word, until an ``end-of-sentence'' (EOS) word is generated.

  

